Spatter: A Tool for Evaluating Gather / Scatter Performance

This paper describes a new benchmark tool, Spatter, for assessing memory system architectures in the context of a specific category of indexed accesses known as gather and scatter. These types of operations are increasingly used to express sparse and irregular data access patterns, and they have widespread utility in many modern HPC applications including scientific simulations, data mining and analysis computations, and graph processing. However, many traditional benchmarking tools like STREAM, STRIDE, and GUPS focus on characterizing only uniform stride or fully random accesses despite evidence that modern applications use varied sets of more complex access patterns. Spatter is an open-source benchmark that provides a tunable and configurable framework to benchmark a variety of indexed access patterns, including variations of gather/scatter that are seen in HPC mini-apps evaluated in this work. The design of Spatter includes tunable backends for OpenMP and CUDA, and experiments show how it can be used to evaluate 1) uniform access patterns for CPU and GPU, 2) prefetching regimes for gather/scatter, 3) compiler implementations of vectorization for gather/scatter, and 4) trace-driven "proxy patterns" that reflect the patterns found in multiple applications. The results from Spatter experiments show that GPUs typically outperform CPUs for these operations, and that Spatter can better represent the performance of some cache-dependent mini-apps than traditional STREAM bandwidth measurements.

==> sections/artifact_description.tex <==


 \small\url{https://github.com/SC-Tech-Program/Author-Kit/blob/master/AD-AE-AppendixForm.pdf}



Summarize the experiments reported in the paper and how they were run. (Example: We ran the NAS Parallel Benchmarks v3.3.1 on NERSC's Cori supercomputer with both Cray's version of MPICH 3.2.1 and with our SuperPGAS communication layer (v0.2), as described in the paper.). MathJax is enabled so you can enter LaTeX mathematical notation within 

\begin{itemize}
\item The characterization study in Section 2 was done using a QEMU trace-driven emulator to run the DoE mini-apps and extract relevant gather / scatter patterns.
\item Three primary sets of experiments were run for this paper: 1) platform comparisons on multiple CPU and GPU platforms using Spatter and BabelStream. 2) SIMD and scalar experiments run on four platforms using Spatter 3) Proxy trace experiments that were run using native DoE mini-apps (AMG and Nekbone) on two platforms, Broadwell and Skylake (Section 5.3). 
\item Babelstream 3.3 is run using a script we have included in our Spatter code repository. This test is used as the baseline "peak bandwidth" for many of our result plots. 
\item Spatter is built using CMake and then is run either by calling the executable with at least a length (amount of data to be moved) and optionally a backend language, device, and platform (for OpenCL). A simple Spatter run can be performed by specifying just a few simple command-line parameters. "./spatter -l 4194304 -s 2 -k scatter -v 4"
\item Since we have run many different backends and variations of the Spatter benchmark, we have endeavored to include scripts in our results and data repository to rerun the experiments. We plan to update these scripts for revisions and if the paper is accepted to help provide usage examples for readers and for replication. 
\end{itemize}




%\scriptsize
%\begin{lstlisting}[linewidth=\columnwidth,label={lst:spatter},caption={Spatter Execution}]
%#Run scatter with 4194304 elements, stride of 2, 
%#and vector width of 4
%
%...
%Warning: No backend specified, guessing OpenMP
%Warning: Kernel file unspecified, guessing kernels/kernels_vector.cl
%backend kernel op time source_size target_size idx_size \\
%worksets bytes_moved usable_bandwidth omp_threads vector_len block_dim
%=======================================================
%OPENMP SCATTER COPY 0.009470 33554432 67108864 33554432 1 67108864 6758.427812 8 4 1 0
%OPENMP SCATTER COPY 0.006139 33554432 67108864 33554432 1 67108864 %10425.439375 8 4 1 0
%%...
%\end{lstlisting}
%\normalsize

%Since Spatter does not by default report a simple set of max/min/average numbers like STREAM, more analysis and context is required for the user to be able to interpret the results. Two scripts are provided to run a sweep of all the most common vector widths, sparsities, and block sizes. Listing \ref{lst:spatter_scripts} shows how these two scripts are used to run multiple instances of Spatter. These two scripts are used to generate the majority of the results evaluated in Section \ref{sec:results}.

%\scriptsize
%\begin{lstlisting}[linewidth=\columnwidth,label={lst:spatter_scripts},caption={Spatter Scripts}]
%#Run a sweep over common parameters with the OpenMP backend 
%#for scatter, gather, and scatter/gather and label results 
%#for a Broadwell CPU
%./sg-sparse-roofline.sh openmp broadwell-cpu
%...
%#Run a sweep but use randomized indices
%./sg-rdm-roofline.sh openmp broadwell-cpu
%...
%\end{lstlisting}
%\normalsize

%Finally, the Spatter benchmark suite provides R and ggplot2\cite{ggplot2} based scripts that plot the output from individual Spatter runs or the output from included sweep scripts. The results in this paper are generated primarily with these scripts, and a future goal is to provide an automated path for a user to download the tool suite, compile, run a set of sweep tests, and then easily generate a set of informative plots. 



\textbf{Artifacts Available (AA)}
This section of the form determines eligibility for the Artifacts Available badge. Three outcomes are possible for your paper: (1) it is eligible for both the AA badge and the Student Cluster Competition Reproducibility Challenge; (2) it is eligible for the AA badge, but not the Reproducibility Challenge; (3) it is ineligible for both the badge and the challenge.

\begin{itemize}
\item All author-created software artifacts are maintained in a public repository under an OSI-approved license. We have a Github repo for the main codebase used for this paper, and a specific results repository for the results for this paper. We will plan to publish a Zenodo DOI with each repo with a release for the code (v0.3) and for the results (v0.1).
\end{itemize}


\textbf{Hardware Artifact Availability}
\begin{itemize}
\item There are no author-created hardware artifacts.
\end{itemize}


\textbf{Data Artifact Availability}
	
\begin{itemize}
\item  All author-created data artifacts are maintained in a public repository under an OSI-approved license.
\end{itemize}

\textbf{Proprietary Artifacts}
\begin{itemize}
\item The traces generated for Spatter proxy trace analysis are created using a proprietary variant of QEMU. As a compromise, we will plan to include the traces used in this paper as inputs that can be used by other researchers for testing and validation.
\item There are no other author created proprietary artifacts. STREAM, LINPACK, and BabelStream are covered by their respective licenses. LINPACK specifically adheres to an Intel license. 
\end{itemize}



\textbf{List of URLs and/or DOIs where artifacts are available} (this information will be unavailable to reviewers, but will be available to the AD/AE Appendices Committee).

\begin{itemize}
\item Codebase (Tagged version 0.3) - \url{https://github.com/hpcgarage/spatter/releases/tag/v0.3}
\item Data and results  \url{https://github.com/hpcgarage/sc19\_spatter}
\end{itemize}


Baseline experimental setup, and modifications made for the paper. Fill in whatever is relevant to your paper and leave the rest blank.
\begin{itemize}
\item Spatter was created from scratch for this paper, so it has not been modified. We have used different compilers, primarily Intel compilers for Intel platforms and Cray compilers for the vectorization studies 
\end{itemize}


Relevant hardware details, e.g., system names, makes, models, and key components such as CPUs, accelerators, and filesystems.
	
\textbf{Operating systems and versions} 
\begin{itemize}
\item This work uses Linux and primarily is run on Ubuntu 16.04 systems and RHEL 7.5 systems.
\end{itemize}


\textbf{Compilers and versions (e.g., "Clang++ v6.0")}
cmake version 3.8 or higher (varies by platform
icc 19.0.3.199
cce version 8.7.10 and 9.0
IBM XL 16.1 
nvcc version 9.1

	
\textbf{Applications and versions} (e.g., "NAMD v2.13" or "SPEC CPU2017")

\begin{itemize}
\item AMG , Github commit 09fe8a7, Feb. 2018
\item Nekbone 2.3.5
\item Lulesh 2.0.3
\item PENNANT 0.9
\item STREAM, v5.10
\item BabelStream, v3.3
\item LINPACK, Intel-2018.3.011
\end{itemize}


\textbf{Libraries and versions} (e.g., "OpenMPI v3.1.0")

\begin{itemize}
\item OpenMP 4.0
\item CUDA 9.1
\end{itemize}

	
\textbf{Key algorithms}
\begin{itemize}
\item Scatter/gather
\end{itemize}

	
\textbf{Input datasets and versions}
\begin{itemize}
\item The proxy traces used for the proxy G/S experiments will be added to the data repo, once we figure out an appropriate way to share them (as they are somewhat large). 
\item All other Spatter runs used synthetically generated data.
\end{itemize}

	
\textbf{Modifications made for the paper: describe how the hardware and software listed in the previous section was improved or otherwise altered.}
\begin{itemize}
\item The primary modifications made to existing software is to compile with different compilers including icc, XL, or cce rather than the default GNU compilers for STREAM and BabelStream
\item In some cases, numactl or likwid-pin were used to limit execution of Spatter to one socket on a particular platform.
\item Most OpenMP tests used OpenMP environment variables specified in the experimental setup to limit execution to one socket or in some cases to one thread.
\end{itemize}

\textbf{Output from commands that gather execution environment information}

Since we have used many different platforms in this evaluation, we have included the output of the provided SC19 script as part of our data repo at \url{https://github.com/hpcgarage/sc19_spatter/tree/master/artifact_descr/exe_environments}.


==> sections/artifact_evaluation.tex <==
\section{Artifact Evaluation}
Discuss the steps taken to help ensure the computational artifacts and results are trustworthy.

Describe controls your team put in place, statistics gathered, or other measures to make the measurements and analyses robust to variability and unknowns in the system. E.g., validation of accuracy and precision of timings, use of manufactured solutions or spectral properties, accounting for aleatoric and epistemic uncertainties, sensitivity of results to initial conditions, sensitivity to parameters and computational environment. Did you perform verification and validation studies? MathJax is enabled so you can enter LaTeX mathematical notation within or 

\textbf{Are you completing an Artifact Evaluation (AE) Appendix?}
No

\textbf{Artifacts Evaluation - Describe if and how you:}
\begin{itemize}
\item Performed verification and validation studies:
\item Validated the accuracy and precision of timings:
\item Used manufactured solutions or spectral properties:
\item  Quantified the sensitivity of your results to initial conditions and/or parameters of the computational environment:
\item  Describe controls, statistics, or other steps taken to make the measurements and analyses robust to variability and unknowns in the system.
\end{itemize}


==> sections/discussion.tex <==

%commented out all old text - in fact, lets remove this section altogether. All text goes in the Results section
\begin{comment}

\section{Discussion} \label{sec:disc}

The results from our initial Spatter benchmarking should not be considered conclusive as to which system is best for sparse operations like \gatherscatter~, but they do point to a few key initial insights that can be used to guide further explorations. 

Overall, newer GPU systems show a separation from CPU and KNL systems in terms of (1) peak effective sparse bandwidth and (2) performance degradation as sparsity increases. Some speculation that would require further experimentation and profiling might be that GPUs are good at coalescing strided loads or that each SM ``core'' has limited cache and thus suffers a smaller performance hit with sparse accesses.
In fact, results from the random indices experiments (Figure \ref{fig:cuda_random}) indicate that both of these hardware features might play a role, as GPUs show a consistent lower bound of effective sparse bandwidth (that does not vary with sparsity) whereas CPUs continue to suffer performance penalties as sparsity increases. 

For CPU-based Spatter results, it is interesting to see that the Skylake and Power9 perform very well when compared to their ``peak'' STREAM bandwidths while the Arm-based TX2 system seems to underperform compared to the other CPU and KNL systems. In particular, the poor results for TX2 and KNL point out that hardware and compiler support for vectorization is important not only to improve \gatherscatter performance, but in the case of KNL to improve ILP for small accesses.
Future work will investigate the effects of additional OpenMP directives to tune for vector widths and testing on new vector-based hardware, such as ARM's Scalable Vector Extensions (SVE). SVE can support hardware implementations from 128 to 2048 bits at 128-bit increments (as opposed to the current 128-bit NEON vector extensions), and we expect that this addition will help to improve the performance of gather and scatter on Arm-based platforms.

The investigation in \Cref{sec:app_char} shows that locality and internal locality in patterns can be important to accurately create a proxy trace for \gatherscatter operations in an application kernel. We also point out that in addition to the stride patterns within \GS instructions, the strides between instructions are also important.

As an example, the selected Nekbone kernel exhibits patterns consisting of $99.96\%$ stride-6 (elements) gathers, while the deltas between instructions are more varied and are often negative: $33.3\%$ are -$1$, and $16.7\%$ are -$5$. 
These negative deltas are important with respect to memory access locality, as they denote reuse of data already in cache, and thus improve performance. Testing on an Intel Broadwell E5 2698 at 2.2 GHz with DDR4-2400 memory using the serial Spatter backend shows the replay of Nekbone patterns using the observed stride between instructions results in 5\% more performance than a pure stride-6 pattern.
Patterns from AMG are more complex than those seen in Nekbone and show an even larger difference; using AMG patterns including observed strides between instructions results in 8\% more performance when compared to using a constant stride-1 between instructions.
\end{comment}

==> sections/pattern.tex <==


\subsubsection{Bandwidth Bandwidth Plots}

\begin{figure}[!htpb]
\centering
\begin{tabular}{c}
\includegraphics[width=1\linewidth]{fig/bwbw/bwbw_Gather.pdf} \\
\textbf{(a)} \\
\includegraphics[width=1\linewidth]{fig/bwbw/bwbw_Scatter.pdf} \\
\textbf{(b)} \\
\end{tabular}
\captionof{figure}{\small Bandwidth-Bandwidth Plots \textmd{\\We display a quantitative ranking of the selected platforms by plotting their pattern bandwidths as a function of the platform's stride-1 bandwidth. For a given platform, it stride-1 bandwidth is on the x=y diagonal, and selected pattern bandwidths appear directly below.} }
\label{fig:bwbw}
\end{figure}

\subsubsection{Radar Plots}

\begin{figure*}
  \includegraphics[width=.98\textwidth,height=.98\textheight,keepaspectratio]{fig/radar/sm2_gather.pdf}
  \caption{This shows some neat radar plots.}
  \label{fig:radar_gather}

\end{figure*}

%% TODO why doesn't this draw?
%\begin{figure}[!htpb]
\begin{figure}
%\includegraphics[width=0.6\textwidth]{fig/radar/sm2_scatter.pdf}
%\centering
\includegraphics[width=0.5\textwidth]{fig/radar/sm2_scatter.pdf}
\caption{Scatter radar plots}
\label{fig:radar_scatter}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}{}
\centering
\caption{Spatter Results for Mini-apps}
\label{table:app-trace}
\begin{small}
\begin{tabular}{l}
\toprule
   Removing this table breaks the document \\

\bottomrule
\end{tabular}
\end{small}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sections/proxy_results.tex <==

\section{Using Proxy \GS to Characterize Mini-apps}
\label{ssec:apptrace}
\begin{table*}
\centering
\caption{Proxy Trace Comparison for the AMG and Nekbone Mini-apps}
\label{table:app-trace}
\begin{small}
\begin{tabular}{l|lrrr|ccc}
\toprule
   \textbf{Application} (FoM) Size & Test Case  & Broadwell & Skylake & Percent  & L1 Miss  & L2 Miss & L3 Miss\\
    &  &  &  & Improvement & BDW / SKX & BDW / SKX & BDW / SKX\\
\midrule
  \textbf{STREAM} (GB/s) & & 17.6 & 10.6 & -39.8 & - & - & -\\
  \textbf{LINPACK} (FLOPS) & & 40.8 & 94.5 & 131.6 & - & - & -\\
\midrule
  \textbf{AMG} (ms) & Native & 149.3 & 108.0 & 27.7 & - & - & -\\
  n = 36 & Spatter &  23.6 & 16.6 & 35.6 & 39.1 / 1115.1   & 67.3 / 35.7  & 824.62 / 11.6 \\

  %n = 36 & Spatter & 98.8 & 93.8  & 5.1 &1.03 / 1.06  &1.85 / 1.63  &139.57 / 8.59 \\
\midrule
     \textbf{Nekbone} (ms) & Native & 440 & 325 & 26.1 & - & - & -\\
    n = 6 & Spatter & 15.4 & 9.9 & 35.8 & 14.4 / 828.5  & 8.10 / 6.40  & $5.9\mathrm{e}{-4}$ / $4.6\mathrm{e}{-3}$ \\
    %n = 6 & Spatter & 244 & 212 & 12.9 &5.14 / 5.16  & 12.53 / 11.41  &141,960 / 16,016 \\
\bottomrule
\end{tabular}
\end{small}
\end{table*}

We next look at an additional set of experiments to investigate whether the application patterns we have generated can be used \textit{to help predict the performance of hot kernels with \GS better than other metrics like STREAM or LINPACK}. 

\textbf{Experimental Setup:} This set of tests uses Spatter's optional PAPI support with PAPI 5.7.0, and it compares two of the previously discussed mini-app kernels, AMG and NEKBONE, with native and Spatter execution on the Broadwell and Skylake test platforms, BDW2 and SKX2 (\cref{table:exp-systems}).  All mini-apps, STREAM, LINPACK, and Spatter are compiled using the locally installed Intel 19.0 tools, as opposed to the Cray compiler tools used for the earlier experiments. The OpenMP backend and one thread are used for all tests, and Spatter, STREAM, and LINPACK results are compared with single-threaded results from the native hot kernels. The Spatter patterns that are used for this test attempt to move the same amount of data as the real mini-app's hot kernels and use the same exact ratio of specific \gatherscatter patterns. In a sense, Spatter's pattern inputs attempt to provide a \textit{spatial-locality proxy} for the actual memory trace from the native mini-app. 

\Cref{table:app-trace} shows results for running Spatter with patterns from the AMG and Nekbone mini-apps natively and with Spatter. Timing is reported in milliseconds for the Native and Spatter execution.  Interestingly, the Skylake core is 40\% slower than the Broadwell core at running STREAM but 132\% faster at running LINPACK. The Skylake system is 27.7\% faster than the Broadwell system at running the native AMG kernel (labeled Percent Improvement) and 26.1\% faster at running the Nekbone kernel. The Spatter proxy trace run predicts that AMG would be 35.65\% faster on the Skylake system and that Nekbone would be 35.8\% faster on Skylake. These results indicate that while STREAM and LINPACK can provide rough indicators of memory system performance and FLOPS, they are not necessarily good figures of merit (FoM) for kernels that include large numbers of \gatherscatter operations.

In addition to timing results for Spatter and the mini-app kernels, we look at PAPI counters for both native and Spatter execution, with a focus on the following events: \texttt{PAPI\_L1\_TCM}, \texttt{PAPI\_L2\_TCM}, \texttt{PAPI\_L3\_TCM}. Our experimentation focuses on whether Spatter can represent the \textbf{ratio of cache misses} for a specific test platforms, where 1 is the ideal result (i.e., no difference in cache misses between Spatter and native execution).
For both AMG and Nekbone, the results for Spatter cache miss ratios vary widely across both platforms with over-predictions that range from one order of magnitude (e.g., L2 miss ratio for NEKBONE at 8.10x and 6.4x) to multiple orders of magnitude (e.g., L1 miss ratios for SKX for both mini-apps at 1115.1x and 828.5x). 

The results from this set of experiments illustrate two important points. First, Spatter can currently potentially predict some relative timing improvements across systems that may be hard to capture with just STREAM. Secondly, the widely varied PAPI cache miss results with Spatter indicate that more complex, higher-order patterns-of-patterns may be needed to accurately represent spatial locality when representing a pattern with Spatter. That is, if an application kernel performs a \gatherscatter pattern and then begins the next iteration of the pattern within the data set already established in the caches, it may have added locality that is not currently represented by repeating the first-order patterns (described in \Cref{sec:app_char}) across new data each time. The resulting added locality can contribute to a significant overestimation of cache misses. Additionally, Spatter does not yet represent \textit{temporal locality}, which is a key component of cache misses. Both of these two sources of error are components of improving Spatter for use as a proxy and are discussed in \cref{sec:futurework}.

==> style/comments.tex <==
%%% Macros to allow authors to make comments in-line in the text
%%% Modified by Jeff Young, 12/14/17
%%% To use: \jsy{This is a comment that should show up in-line in the text}

% For more advanced color handling
\usepackage{xcolor}
\usepackage{amssymb}

\usepackage{comment}


%Comment for Jeff
\newcommand{\remjy}[1]{\marginpar{\textcolor{orange}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{orange}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamejy}[2]{{\marginpar{\textcolor{orange}{$\star$ #2}}\sf{\normalsize{\textcolor{orange}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\jsy}[1]{\remnamejy{#1}{jsy}}

%Comment for Patrick
\newcommand{\rempl}[1]{\marginpar{\textcolor{blue}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamepl}[2]{{\marginpar{\textcolor{blue}{$\star$ #2}}\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\pl}[1]{\remnamepl{#1}{pl}}

%Comment for Rich
\newcommand{\remrv}[1]{\marginpar{\textcolor{blue}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnamerv}[2]{{\marginpar{\textcolor{blue}{$\star$ #2}}\sf{\normalsize{\textcolor{blue}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\rv}[1]{\remnamerv{#1}{rv}}

%Comment for Aaron
\newcommand{\remav}[1]{\marginpar{\textcolor{red}{$\blacktriangleleft$}}{\sf{\normalsize{\textcolor{red}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\remnameav}[2]{{\marginpar{\textcolor{red}{$\star$ #2}}\sf{\normalsize{\textcolor{red}{$\blacksquare$\em{ #1} $\blacksquare$}}}}}
\newcommand{\av}[1]{\remnameav{#1}{av}}

